The Recurrent Transformer: Greater Effective Depth and Efficient Decoding

Transformers process tokens in parallel but are temporally shallow: at position $t$, each layer attends to key-value pairs computed based on the previous layer, yielding a depth capped by the number of layers. Recurrent models offer unbounded temporal depth but suffer from optimization instability and historically underutilize modern accelerators. We introduce the Recurrent Transformer, a simple architectural change where each layer attends to key-value pairs computed off its own activations, yielding layerwise recurrent memory while preserving standard autoregressive decoding cost. We show that the architecture can emulate both (i) a conventional Transformer and (ii) token-to-token recurrent updates under mild assumptions, while avoiding optimization instability. Naively, prefill/training appears bandwidth-bound with effective arithmetic intensity near $1$ because keys and values are revealed sequentially; we give an exact tiling-based algorithm that preserves the mathematical computation while reducing HBM traffic from $\Theta(N^2)$ to $\Theta(N\log N)$, increasing effective arithmetic intensity to $\Theta(N/\log N)$ for sequence length $N$. On 150M and 300M parameter C4 pretraining, Recurrent Transformers improve cross-entropy over a parameter-matched Transformer baseline and achieve the improvement with fewer layers (fixed parameters), suggesting that recurrence can trade depth for width, thus reducing KV cache memory footprint and inference latency.

==> tables/c4_512_300m_table.tex <==
\begin{table}[t]
\centering
\caption{C4 pretraining loss for 300M parameter model.\alex{since the main claims are about depth, i would sort this table by num layers, and then bold the best val ce vals. also maybe it would be nice to have this + figure 1 as the main "figure", so left plot is the current fig 2, right col is table 1}}
\label{tab:c4-512-300m}
\begin{tabular}{lccc}
\toprule
Model & Layers & Width & Val CE $\downarrow$ \\
\midrule
Transformer & 6 & $2048$ & $2.917$ \\
Transformer & 12 & $1408$ & $2.896$ \\
Transformer & 24 & $1024$ & $2.892$ \\
\methodname{} & 12 & $1408$ & $2.867$ \\
\methodname{} & 6 & $2048$ & $2.86$ \\
\bottomrule
\end{tabular}
\end{table}
